ToF-SIMS Investigations on Dental Implant Materials and Adsorbed Protein Films

In this work the two experimental dental implant materials FAT and FAW, made of fluoroapatite particles embedded in polymer matrices, and films of the proteins lysozyme, amylase and bovine serum albumin (BSA), adsorbed to the two dental implant materials, were investigated with time-of-flight secondary ion mass spectrometry (ToF-SIMS) and the multivariate data analysis technique discriminant principal component analysis (DPCA).

==> Fdistribution.tex <==
{{\def\dash{\raise2.1pt\hbox{\rule{5pt}{0.3pt}}\hspace{1pt}}\begin{tabbing}
{\textbf{function}}\hspace{6pt}ausgabe=Fdistribution(n)
\\
{\it{\%ausgabe=Fdistribution(n)}}\\
{\it{\%finds\hspace{6pt}the\hspace{6pt}upper\hspace{6pt}limit\hspace{6pt}of\hspace{6pt}the\hspace{6pt}95\%\hspace{6pt}confidence\hspace{6pt}interval}}\\
{\it{\%of\hspace{6pt}an\hspace{6pt}F\hspace{6pt}distribution\hspace{6pt}for\hspace{6pt}2\hspace{6pt}variables\hspace{6pt}and\hspace{6pt}n\hspace{6pt}measurements;
}}\\
{\it{\%values\hspace{6pt}are\hspace{6pt}from\hspace{6pt}the\hspace{6pt}table\hspace{6pt}in\hspace{6pt}J.E.\hspace{6pt}Jackson,\hspace{6pt}A\hspace{6pt}user{'}s\hspace{6pt}guide\hspace{6pt}}}\\
{\it{\%to\hspace{6pt}principal\hspace{6pt}components,\hspace{6pt}John\hspace{6pt}Wiley\hspace{6pt}and\hspace{6pt}sons,\hspace{6pt}New\hspace{6pt}York,1991;}}\\
{\it{\%intermedial\hspace{6pt}values\hspace{6pt}linearly\hspace{6pt}approximated
}}\\

\\
{\it{\%tabulated\hspace{6pt}values:
}}\\
F=\hspace{6pt}{[}1.9950000e+002
\\
\hspace{12pt}1.9000000e+001
\\
\hspace{12pt}9.5500000e+000
\\
\hspace{12pt}6.9400000e+000
\\
\hspace{12pt}5.7900000e+000
\\
\hspace{12pt}5.1400000e+000
\\
\hspace{12pt}4.7400000e+000
\\
\hspace{12pt}4.4600000e+000
\\
\hspace{12pt}4.2600000e+000
\\
\hspace{12pt}4.1000000e+000
\\
\hspace{12pt}3.9800000e+000
\\
\hspace{12pt}3.8900000e+000
\\
\hspace{12pt}3.8100000e+000
\\
\hspace{12pt}3.7400000e+000
\\
\hspace{12pt}3.6800000e+000
\\
\hspace{12pt}3.6300000e+000
\\
\hspace{12pt}3.5900000e+000
\\
\hspace{12pt}3.5500000e+000
\\
\hspace{12pt}3.5200000e+000
\\
\hspace{12pt}3.4900000e+000
\\
\hspace{12pt}3.4700000e+000
\\
\hspace{12pt}3.4400000e+000
\\
\hspace{12pt}3.4200000e+000
\\
\hspace{12pt}3.4000000e+000
\\
\hspace{12pt}3.3900000e+000
\\
\hspace{12pt}3.3700000e+000
\\
\hspace{12pt}3.3500000e+000
\\
\hspace{12pt}3.3400000e+000
\\
\hspace{12pt}3.3300000e+000
\\
\hspace{12pt}3.3200000e+000
\\
\hspace{12pt}3.2300000e+000
\\
\hspace{12pt}3.1500000e+000
\\
\hspace{12pt}3.0700000e+000
\\
\hspace{12pt}3.0000000e+000{]};
\\
\\
{\it{\%to\hspace{6pt}find\hspace{6pt}the\hspace{6pt}right\hspace{6pt}value\hspace{6pt}the\hspace{6pt}number\hspace{6pt}of\hspace{6pt}measurements\hspace{6pt}has}}\\
{\it{\%to\hspace{6pt}be\hspace{6pt}reduced\hspace{6pt}by\hspace{6pt}the\hspace{6pt}number\hspace{6pt}of\hspace{6pt}variables:
}}\\
n=n\dash{}2;
\\

\\
{\textbf{if}}\hspace{6pt}n\hspace{6pt}$<$1
\\
\hspace{36pt}disp({\texttt{{'}Error:\hspace{6pt}Number\hspace{6pt}of\hspace{6pt}measurements\hspace{6pt}must\hspace{6pt}be\hspace{6pt}greater\hspace{6pt}2!{'}}})
\\
\hspace{36pt}
\\
\hspace{12pt}{\textbf{elseif}}\hspace{6pt}n$<$31
\\
\hspace{48pt}
\\
\hspace{48pt}{\it{\%the\hspace{6pt}first\hspace{6pt}30\hspace{6pt}values\hspace{6pt}correspond\hspace{6pt}to\hspace{6pt}1\hspace{6pt}to\hspace{6pt}30\hspace{6pt}measurements:
}}\\
\hspace{48pt}ausgabe=F(n);
\\
\hspace{48pt}
\\
\hspace{24pt}{\textbf{elseif}}\hspace{6pt}n$<$40
\\
\hspace{48pt}
\\
\hspace{48pt}{\it{\%linear\hspace{6pt}interpolation:
}}\\
\hspace{48pt}ausgabe=3.32\dash{}(n\dash{}30)$\ast$0.009;
\\
\hspace{48pt}
\\
\hspace{24pt}{\textbf{elseif}}\hspace{6pt}n$<$60
\\
\hspace{48pt}ausgabe=3.23\dash{}(n\dash{}40)$\ast$0.004;
\\
\hspace{48pt}
\\
\hspace{24pt}{\textbf{elseif}}\hspace{6pt}n$<$121
\\
\hspace{48pt}ausgabe=3.15\dash{}(n\dash{}60)$\ast$8/6000;
\\
\hspace{48pt}
\\
\hspace{24pt}{\textbf{elseif}}\hspace{6pt}n$>$120
\\
\hspace{36pt}disp({\texttt{{'}Warning:\hspace{6pt}Using\hspace{6pt}approximation\hspace{6pt}for\hspace{6pt}(number\hspace{6pt}of\hspace{6pt}measurements)\hspace{6pt}$>$$>$\hspace{6pt}120{'}}})
\\
\hspace{36pt}ausgabe=3;
\\
\hspace{30pt}
\\
{\textbf{end}}
\\

\\
\hspace{36pt}
\end{tabbing}}}


==> abstract.tex <==
\begin{abstract}
\textsc{Hier fehlt noch die Zusammenfassung}
\end{abstract}


==> auswahl.tex <==
{{\def\dash{\raise2.1pt\hbox{\rule{5pt}{0.3pt}}\hspace{1pt}}\begin{tabbing}
{\textbf{function}}\hspace{6pt}out=auswahl(in)\\
{\it{\%out=auswahl(in)}}\\
{\it{\%selects\hspace{6pt}amino\hspace{6pt}acid\hspace{6pt}related\hspace{6pt}peaks\hspace{6pt}from\hspace{6pt}unit\hspace{6pt}mass}}\\
{\it{\%mass\hspace{6pt}spectra
}}\\
out(1,:)=in(30,:);\hspace{6pt}{\it{\%Gly
}}\\
out(2,:)=in(43,:);\hspace{6pt}{\it{\%Arg
}}\\
out(3,:)=in(44,:);\hspace{6pt}{\it{\%Ala
}}\\
out(4,:)=in(45,:);\hspace{6pt}{\it{\%Cys
}}\\
out(5,:)=in(60,:);\hspace{6pt}{\it{\%Ser
}}\\
out(6,:)=in(61,:);\hspace{6pt}{\it{\%Met
}}\\
out(7,:)=in(68,:);\hspace{6pt}{\it{\%Pro
}}\\
out(8,:)=in(69,:);\hspace{6pt}{\it{\%Thr
}}\\
out(9,:)=in(70,:);\hspace{6pt}{\it{\%Asn,\hspace{6pt}Pro
}}\\
out(10,:)=in(71,:);\hspace{6pt}{\it{\%Ser
}}\\
out(11,:)=in(72,:);\hspace{6pt}{\it{\%Val
}}\\
out(12,:)=in(73,:);\hspace{6pt}{\it{\%Arg
}}\\
out(13,:)=in(74,:);\hspace{6pt}{\it{\%Thr
}}\\
out(14,:)=in(81,:);\hspace{6pt}{\it{\%His
}}\\
out(15,:)=in(82,:);\hspace{6pt}{\it{\%His
}}\\
out(16,:)=in(83,:);\hspace{6pt}{\it{\%Val
}}\\
out(17,:)=in(84,:);\hspace{6pt}{\it{\%Gln,\hspace{6pt}Glu,\hspace{6pt}Lys
}}\\
out(18,:)=in(86,:);\hspace{6pt}{\it{\%Ile,\hspace{6pt}Leu
}}\\
out(19,:)=in(87,:);\hspace{6pt}{\it{\%Asn
}}\\
out(20,:)=in(88,:);\hspace{6pt}{\it{\%Asn,\hspace{6pt}Asp
}}\\
out(21,:)=in(98,:);\hspace{6pt}{\it{\%Asn
}}\\
out(22,:)=in(100,:);\hspace{6pt}{\it{\%Arg
}}\\
out(23,:)=in(101,:);\hspace{6pt}{\it{\%Arg
}}\\
out(24,:)=in(102,:);\hspace{6pt}{\it{\%Glu
}}\\
out(25,:)=in(107,:);\hspace{6pt}{\it{\%Tyr
}}\\
out(26,:)=in(110,:);\hspace{6pt}{\it{\%His
}}\\
out(27,:)=in(112,:);\hspace{6pt}{\it{\%Arg
}}\\
out(28,:)=in(120,:);\hspace{6pt}{\it{\%Phe
}}\\
out(29,:)=in(127,:);\hspace{6pt}{\it{\%Arg
}}\\
out(30,:)=in(130,:);\hspace{6pt}{\it{\%Trp
}}\\
out(31,:)=in(131,:);\hspace{6pt}{\it{\%Phe
}}\\
out(32,:)=in(136,:);\hspace{6pt}{\it{\%Tyr
}}\\
out(33,:)=in(159,:);\hspace{6pt}{\it{\%Trp
}}\\
out(34,:)=in(170,:);\hspace{6pt}{\it{\%Trp}}
\end{tabbing}}}


==> dpca.tex <==
{{\def\dash{\raise2.1pt\hbox{\rule{5pt}{0.3pt}}\hspace{1pt}}\begin{tabbing}
{\textbf{function}}\hspace{6pt}{[}loading,score,variance,varianceintra{]}=dpca(x,anz,rep)\\
{\it{\%{[}loading,score,relvariance,varianceintra{]}=dpca(x,anz,rep)}}\\
{\it{\%performs\hspace{6pt}discriminant\hspace{6pt}principal\hspace{6pt}component\hspace{6pt}analysis}}\\
{\it{\%x:\hspace{6pt}(mxn)\dash{}matrix:\hspace{6pt}values\hspace{6pt}of\hspace{6pt}m\hspace{6pt}variables\hspace{6pt}for\hspace{6pt}n\hspace{6pt}measurements}}\\
{\it{\%anz:\hspace{6pt}number\hspace{6pt}of\hspace{6pt}groups}}\\
{\it{\%rep:\hspace{6pt}(1xanz)\dash{}vector:\hspace{6pt}number\hspace{6pt}of\hspace{6pt}measurements\hspace{6pt}per\hspace{6pt}group}}\\
{\it{\%loading:\hspace{6pt}(mxm)\dash{}matrix:\hspace{6pt}loadings\hspace{6pt}of\hspace{6pt}m\hspace{6pt}DPC\hspace{6pt}as\hspace{6pt}m\hspace{6pt}columns}}\\
{\it{\%score:\hspace{6pt}(mxn)\dash{}matrix:\hspace{6pt}scores\hspace{6pt}of\hspace{6pt}m\hspace{6pt}DPC\hspace{6pt}for\hspace{6pt}n\hspace{6pt}measurements}}\\
{\it{\%variance:\hspace{6pt}(1xm)\dash{}vector:\hspace{6pt}variance\hspace{6pt}captured\hspace{6pt}by\hspace{6pt}the\hspace{6pt}m\hspace{6pt}DPC}}\\
{\it{\%varianceintra:\hspace{6pt}(mx1)\dash{}vector:\hspace{6pt}pooled\hspace{6pt}intra\hspace{6pt}group\hspace{6pt}variances\hspace{6pt}of\hspace{6pt}m\hspace{6pt}variables}}\\
{\it{\%for\hspace{6pt}details\hspace{6pt}on\hspace{6pt}the\hspace{6pt}PCA\hspace{6pt}algorithm\hspace{6pt}see\hspace{6pt}J.\hspace{6pt}Shlens,\hspace{6pt}}}\\
{\it{\%A\hspace{6pt}tutorial\hspace{6pt}on\hspace{6pt}principal\hspace{6pt}component\hspace{6pt}analysis,\hspace{6pt}10/12/2005}}\\
{\it{\%for\hspace{6pt}details\hspace{6pt}on\hspace{6pt}DPCA\hspace{6pt}see\hspace{6pt}P.W.\hspace{6pt}Yendle,\hspace{6pt}H.J.M.\hspace{6pt}Macfie,}}\\
{\it{\%Discriminant\hspace{6pt}principal\hspace{6pt}components\hspace{6pt}analysis,}}\\
{\it{\%J.\hspace{6pt}of\hspace{6pt}Chemometrics\hspace{6pt}3,\hspace{6pt}589\dash{}600,\hspace{6pt}1989
}}\\

\\
{[}m,n{]}=size(x);
\\
{[}sizerepx,sizerepy{]}=size(rep);
\\
{\textbf{if}}\hspace{6pt}sizerepy==1
\\
\hspace{24pt}rep=repmat(rep,1,anz);
\\
{\textbf{end}}
\\

\\
{\it{\%scaling\hspace{6pt}by\hspace{6pt}total\hspace{6pt}intensity:
}}\\
{\textbf{for}}\hspace{6pt}k=1:n
\\
\hspace{24pt}x(:,k)=x(:,k)/sum(x(:,k));
\\
{\textbf{end}}
\\
\\
{\it{\%pooled\hspace{6pt}intra\hspace{6pt}group\hspace{6pt}variances\hspace{6pt}of\hspace{6pt}the\hspace{6pt}variables:
}}\\
{\it{\%\dash{}$>$\hspace{6pt}varianceintra:\hspace{6pt}(mx1)
}}\\
varianceintra=zeros(m,1);
\\
{\textbf{for}}\hspace{6pt}k=1:m
\\
\hspace{24pt}start=1;
\\
\hspace{24pt}stop=0;
\\
\hspace{24pt}{\textbf{for}}\hspace{6pt}o=1:anz
\\
\hspace{48pt}stop=stop+rep(o);
\\
\hspace{48pt}varianceintra(k)=varianceintra(k)+var(x(k,start:stop));
\\
\hspace{48pt}start=start+rep(o);
\\
\hspace{24pt}{\textbf{end}}
\\
{\textbf{end}}
\\
\\
{\it{\%scaling\hspace{6pt}by\hspace{6pt}intra\hspace{6pt}group\hspace{6pt}standard\hspace{6pt}deviations:}}\\
{\it{\%\dash{}$>$\hspace{6pt}scaled\hspace{6pt}data\hspace{6pt}matrix\hspace{6pt}s
}}\\
{\textbf{for}}\hspace{6pt}k=1:m
\\
\hspace{24pt}s(k,:)=x(k,:)/sqrt(varianceintra(k));
\\
{\textbf{end}}
\\
\\
{\it{\%scaled\hspace{6pt}group\hspace{6pt}means:}}\\
{\it{\%\dash{}$>$\hspace{6pt}(mxanz)\dash{}matrix\hspace{6pt}sbar
}}\\
{\textbf{for}}\hspace{6pt}k=1:m
\\
\hspace{24pt}start=1;
\\
\hspace{24pt}stop=0;
\\
\hspace{24pt}{\textbf{for}}\hspace{6pt}o=1:anz
\\
\hspace{48pt}stop=stop+rep(o);
\\
\hspace{48pt}sbar(k,o)=mean(s(k,start:stop));
\\
\hspace{48pt}start=start+rep(o);
\\
\hspace{24pt}{\textbf{end}}
\\
{\textbf{end}}
\\
\\
{\it{\%(mxn)\dash{}matrix\hspace{6pt}of\hspace{6pt}scaled\hspace{6pt}group\hspace{6pt}means:
}}\\
groupmeans=repmat(sbar(:,1),1,rep(1));
\\
{\textbf{for}}\hspace{6pt}o=2:anz
\\
\hspace{24pt}groupmeans={[}groupmeans\hspace{6pt}repmat(sbar(:,o),1,rep(o)){]};
\\
{\textbf{end}}
\\
\\
{\it{\%PCA\hspace{6pt}with\hspace{6pt}SVD\hspace{6pt}\dash{}$>$\hspace{6pt}(mxm)\dash{}matrix\hspace{6pt}of\hspace{6pt}loadings\hspace{6pt}loading:}}\\
\\
{\it{\%mean\dash{}centering:
}}\\
mn=mean(groupmeans,2);
\\
groupmeans=groupmeans\dash{}repmat(mn,1,n);
\\
helpmatrix=groupmeans{'}/sqrt(n\dash{}1);
\\
{[}u,singularvalues,loading{]}=svd(helpmatrix);
\\

\\
{\it{\%projection\hspace{6pt}\dash{}$>$\hspace{6pt}(mxn)\dash{}matrix\hspace{6pt}of\hspace{6pt}scores\hspace{6pt}score
}}\\
score=loading{'}$\ast$s;
\\

\\
{\it{\%variances\hspace{6pt}of\hspace{6pt}the\hspace{6pt}DPC:}}\\
{\it{\%\dash{}$>$\hspace{6pt}m\dash{}vector\hspace{6pt}variance
}}\\
{\textbf{for}}\hspace{6pt}k=1:m
\\
\hspace{24pt}variance(k)=var(score(k,:));
\\
{\textbf{end}}
\\

\\
{\it{\%saving\hspace{6pt}loadings\hspace{6pt}and\hspace{6pt}scores:
}}\\
save\hspace{6pt}dloading.dat\hspace{6pt}loading\hspace{6pt}\dash{}ascii;
\\
save\hspace{6pt}dscore.dat\hspace{6pt}score\hspace{6pt}\dash{}ascii;
\end{tabbing}}}


==> dpcaprojektion.tex <==
{{\def\dash{\raise2.1pt\hbox{\rule{5pt}{0.3pt}}\hspace{1pt}}\begin{tabbing}
{\textbf{function}}\hspace{6pt}score=dpcaprojektion(loading,varianceintra,data,index,stil)\\
{\it{\%dpcaprojektion(loading,varianceintra,data,index,stil)}}\\
{\it{\%projects\hspace{6pt}a\hspace{6pt}data\hspace{6pt}matrix\hspace{6pt}using\hspace{6pt}DPC\hspace{6pt}loadings\hspace{6pt}into\hspace{6pt}a\hspace{6pt}scores\hspace{6pt}plot}}\\
{\it{\%loading:\hspace{6pt}(mxm)\dash{}matrix:\hspace{6pt}loadings\hspace{6pt}of\hspace{6pt}m\hspace{6pt}DPC\hspace{6pt}as\hspace{6pt}m\hspace{6pt}columns}}\\
{\it{\%varianceintra:\hspace{6pt}(mx1)\dash{}vector:\hspace{6pt}pooled\hspace{6pt}intra\hspace{6pt}group\hspace{6pt}variances\hspace{6pt}of\hspace{6pt}m\hspace{6pt}variables}}\\
{\it{\%data:\hspace{6pt}(mxn)\dash{}matrix:\hspace{6pt}values\hspace{6pt}of\hspace{6pt}m\hspace{6pt}variables\hspace{6pt}for\hspace{6pt}n\hspace{6pt}measurements}}\\
{\it{\%index:\hspace{6pt}number\hspace{6pt}of\hspace{6pt}first\hspace{6pt}displayed\hspace{6pt}DPC\hspace{6pt}in\hspace{6pt}the\hspace{6pt}scores\hspace{6pt}plot}}\\
{\it{\%stil:\hspace{6pt}style\hspace{6pt}of\hspace{6pt}the\hspace{6pt}projected\hspace{6pt}data\hspace{6pt}points}}\\
{\it{\%score:\hspace{6pt}(mxn)\dash{}matrix:\hspace{6pt}projected\hspace{6pt}scores\hspace{6pt}of\hspace{6pt}m\hspace{6pt}DPC\hspace{6pt}for\hspace{6pt}n\hspace{6pt}measurements}}\\
{\it{\%for\hspace{6pt}details\hspace{6pt}on\hspace{6pt}DPCA\hspace{6pt}see\hspace{6pt}P.W.\hspace{6pt}Yendle,\hspace{6pt}H.J.M.\hspace{6pt}Macfie,}}\\
{\it{\%Discriminant\hspace{6pt}principal\hspace{6pt}components\hspace{6pt}analysis,}}\\
{\it{\%J.\hspace{6pt}of\hspace{6pt}Chemometrics\hspace{6pt}3,\hspace{6pt}589\dash{}600,\hspace{6pt}1989
}}\\

\\
{[}m,n{]}=size(data);
\\

\\
{\it{\%scaling\hspace{6pt}of\hspace{6pt}measurements\hspace{6pt}by\hspace{6pt}total\hspace{6pt}intensity:
}}\\
{\textbf{for}}\hspace{6pt}k=1:n
\\
\hspace{24pt}data(:,k)=data(:,k)/sum(data(:,k));
\\
{\textbf{end}}
\\
\\
{\it{\%scaling\hspace{6pt}by\hspace{6pt}pooled\hspace{6pt}intra\hspace{6pt}group\hspace{6pt}variance:
}}\\
{\textbf{for}}\hspace{6pt}k=1:m
\\
\hspace{24pt}scaled(k,:)=data(k,:)/sqrt(varianceintra(k));
\\
{\textbf{end}}\\
\\
{\it{\%projecting:
}}\\
score=loading{'}$\ast$scaled;
\\
\\
{\it{\%plotting\hspace{6pt}can\hspace{6pt}be\hspace{6pt}prevented\hspace{6pt}with\hspace{6pt}style\hspace{6pt}{'}no{'}:
}}\\
{\textbf{if}}\hspace{6pt}stil=={\texttt{{'}no{'}}}
\\
\hspace{24pt}{\textbf{return}}
\\
{\textbf{end}}
\\
\\
{\it{\%plotting:
}}\\
hold\hspace{6pt}on
\\
plot(score(index,:),score(index+1,:),stil);
\end{tabbing}}}


==> einlesen.tex <==
\def\dash{\raise2.1pt\hbox{\rule{5pt}{0.3pt}}
\hspace{1pt}}\begin{tabbing}
{\textbf{function}}\hspace{6pt}out=einlesen(prefix,start,stop,suffix,m)\\
{\it{\%out=einlesen(prefix,start,stop,suffix,m))}}\\
{\it{\%reads\hspace{6pt}the\hspace{6pt}files\hspace{6pt}{'}c:$\backslash$tof\dash{}sims$\backslash$ascii$\backslash$prefixstartsuffix.asc{'}}}\\
{\it{\%to\hspace{6pt}{'}c:$\backslash$tof\dash{}sims$\backslash$ascii$\backslash$prefixstopsuffix.asc{'}\hspace{6pt}containing}}\\
{\it{\%unit\dash{}mass\hspace{6pt}mass\hspace{6pt}spectra\hspace{6pt}exported\hspace{6pt}from\hspace{6pt}WinCadence\hspace{6pt}and}}\\
{\it{\%forms\hspace{6pt}a\hspace{6pt}(mx(stop\dash{}start))\dash{}data\hspace{6pt}matrix\hspace{6pt}with\hspace{6pt}the\hspace{6pt}}}\\
{\it{\%first\hspace{6pt}m\hspace{6pt}masses\hspace{6pt}in\hspace{6pt}(stop\dash{}start)\hspace{6pt}spectra}}\\
\\
longprefix={[}{\texttt{{'}c:$\backslash$tof\dash{}sims$\backslash$ascii$\backslash${'}}},prefix{]};\\
\\
k=start;\\
filename={[}longprefix,int2str(k),suffix,{\texttt{{'}.asc{'}}}{]};\\
\\
{\it{\%reading\hspace{6pt}the\hspace{6pt}first\hspace{6pt}WinCadence\hspace{6pt}export:}}\\
x=load(filename);\\
\\
{\it{\%extracting\hspace{6pt}the\hspace{6pt}counts\hspace{6pt}at\hspace{6pt}the\hspace{6pt}first\hspace{6pt}m\hspace{6pt}masses:}}\\
out=voll(x,m);\\
\\
{\it{\%loop\hspace{6pt}for\hspace{6pt}the\hspace{6pt}other\hspace{6pt}files:}}\\
{\textbf{for}}\hspace{6pt}k=start+1:stop\\
\hspace{24pt}filename={[}longprefix,int2str(k),suffix,{\texttt{{'}.asc{'}}}{]};\\
\hspace{24pt}x=load(filename);\\
\hspace{24pt}{\it{\%new\hspace{6pt}data\hspace{6pt}is\hspace{6pt}appended\hspace{6pt}to\hspace{6pt}the\hspace{6pt}existing\hspace{6pt}data\hspace{6pt}matrix}}\\
\hspace{24pt}out=matrix(out,x);\\
{\textbf{end}}
\end{tabbing}


==> ellipse.tex <==
{{\def\dash{\raise2.1pt\hbox{\rule{5pt}{0.3pt}}\hspace{1pt}}\begin{tabbing}
{\textbf{function}}\hspace{6pt}ellipse(X,Tsquare,color)\\
{\it{\%ellipse(X,Tsquare,color)}}\\
{\it{\%plots\hspace{6pt}a\hspace{6pt}probability\hspace{6pt}ellipse\hspace{6pt}around\hspace{6pt}data\hspace{6pt}points}}\\
{\it{\%X:\hspace{6pt}(2xn)\dash{}matrix\hspace{6pt}containing\hspace{6pt}n\hspace{6pt}measurements\hspace{6pt}of\hspace{6pt}2\hspace{6pt}variables}}\\
{\it{\%Tsquare:\hspace{6pt}critical\hspace{6pt}value\hspace{6pt}of\hspace{6pt}the\hspace{6pt}TSquare\hspace{6pt}distribution}}\\
{\it{\%color:\hspace{6pt}colour\hspace{6pt}(r,b,g,c,m,y\hspace{6pt}or\hspace{6pt}k)}}\\
{\it{\%for\hspace{6pt}details\hspace{6pt}on\hspace{6pt}the\hspace{6pt}algorithm\hspace{6pt}see\hspace{6pt}J.E.\hspace{6pt}Jackson,\hspace{6pt}A\hspace{6pt}user{'}s\hspace{6pt}guide\hspace{6pt}}}\\
{\it{\%to\hspace{6pt}principal\hspace{6pt}components,\hspace{6pt}John\hspace{6pt}Wiley\hspace{6pt}and\hspace{6pt}sons\hspace{6pt}inc.,\hspace{6pt}New\hspace{6pt}York,\hspace{6pt}1991
}}\\

\\
{[}m,n{]}=size(X);
\\
{\textbf{if}}\hspace{6pt}m\~{}=2\hspace{6pt}
\\
\hspace{24pt}fprintf(1,{\texttt{{'}\hspace{6pt}$\backslash$n\hspace{6pt}Error:\hspace{6pt}Data\hspace{6pt}matrix\hspace{6pt}must\hspace{6pt}be\hspace{6pt}2\hspace{6pt}x\hspace{6pt}n!\hspace{6pt}$\backslash$n{'}}});
\\
\hspace{24pt}{\textbf{return}}
\\
{\textbf{end}}
\\

\\
{\it{\%Centre\hspace{6pt}of\hspace{6pt}the\hspace{6pt}ellipse:
}}\\
mitte=mean(X,2);
\\

\\
{\it{\%Mean\dash{}centered\hspace{6pt}auxiliary\hspace{6pt}matrix:
}}\\
Y=X\dash{}repmat(mitte,1,n);
\\
Y=Y{'}/sqrt(n\dash{}1);
\\
\\
{\it{\%singular\hspace{6pt}value\hspace{6pt}decomposition\hspace{6pt}to\hspace{6pt}calculate\hspace{6pt}}}\\
{\it{\%principal\hspace{6pt}components\hspace{6pt}and\hspace{6pt}standard\hspace{6pt}deviations:
}}\\
{[}u,S,PC{]}=svd(Y);
\\

\\
{\it{\%standard\hspace{6pt}deviations:
}}\\
S=diag(S);
\\

\\
{\it{\%rescaling\hspace{6pt}of\hspace{6pt}principal\hspace{6pt}components
}}\\
PC(:,1)=S(1)$\ast$PC(:,1);
\\
PC(:,2)=S(2)$\ast$PC(:,2);
\\

\\
kmax=sqrt(Tsquare);
\\
hold\hspace{6pt}on\\

\\
{\it{\%calculation\hspace{6pt}and\hspace{6pt}plotting\hspace{6pt}of\hspace{6pt}the\hspace{6pt}ellipse;}}\\
{\it{\%number\hspace{6pt}of\hspace{6pt}points\hspace{6pt}can\hspace{6pt}be\hspace{6pt}controlled}}\\
{\it{\%by\hspace{6pt}the\hspace{6pt}stepwidth\hspace{6pt}of\hspace{6pt}the\hspace{6pt}loop:
}}\\
{\textbf{for}}\hspace{6pt}k=0:0.04:kmax
\\
\hspace{24pt}g=k;
\\
\hspace{24pt}h=sqrt(Tsquare\dash{}k\^{}2);
\\
\hspace{24pt}x=mitte+g$\ast$PC(:,1)+h$\ast$PC(:,2);
\\
\hspace{24pt}plot(x(1),x(2),color)
\\
\hspace{24pt}x=mitte+g$\ast$PC(:,1)\dash{}h$\ast$PC(:,2);
\\
\hspace{24pt}plot(x(1),x(2),color)
\\
\hspace{24pt}x=mitte\dash{}g$\ast$PC(:,1)+h$\ast$PC(:,2);
\\
\hspace{24pt}plot(x(1),x(2),color)
\\
\hspace{24pt}x=mitte\dash{}g$\ast$PC(:,1)\dash{}h$\ast$PC(:,2);
\\
\hspace{24pt}plot(x(1),x(2),color)\hspace{36pt}
\\
{\textbf{end}}
\\

\\
g=sqrt(Tsquare);
\\
h=0;
\\
x=mitte\dash{}g$\ast$PC(:,1);
\\
plot(x(1),x(2),color)\hspace{6pt}
\\
x=mitte+g$\ast$PC(:,1);
\\
plot(x(1),x(2),color)\hspace{6pt}
\end{tabbing}}}


==> loo.tex <==
{{\def\dash{\raise2.1pt\hbox{\rule{5pt}{0.3pt}}\hspace{1pt}}\begin{tabbing}
{\textbf{function}}\hspace{6pt}loo(data,anz,rep)
\\
{\it{\%loo(data,anz,rep)}}\\
{\it{\%performs\hspace{6pt}DPCA,\hspace{6pt}leaves\hspace{6pt}each\hspace{6pt}measurement\hspace{6pt}out\hspace{6pt}once}}\\
{\it{\%and\hspace{6pt}projects\hspace{6pt}it\hspace{6pt}into\hspace{6pt}the\hspace{6pt}scores\hspace{6pt}plot}}\\
{\it{\%data:\hspace{6pt}(mxn)\hspace{6pt}matrix:\hspace{6pt}values\hspace{6pt}of\hspace{6pt}m\hspace{6pt}variables\hspace{6pt}in\hspace{6pt}n\hspace{6pt}measurements}}\\
{\it{\%anz:\hspace{6pt}number\hspace{6pt}of\hspace{6pt}groups}}\\
{\it{\%rep:\hspace{6pt}(anz)\dash{}vector:\hspace{6pt}number\hspace{6pt}of\hspace{6pt}measurements\hspace{6pt}per\hspace{6pt}group\hspace{6pt}
}}\\

\\
{[}m,n{]}=size(data);
\\

\\
{[}sizerepx,sizerepy{]}=size(rep);
\\
{\textbf{if}}\hspace{6pt}sizerepy==1
\\
\hspace{24pt}rep=repmat(rep,1,anz);
\\
{\textbf{end}}
\\

\\
{\it{\%loop\hspace{6pt}to\hspace{6pt}leave\hspace{6pt}out\hspace{6pt}one\hspace{6pt}measurement\hspace{6pt}after\hspace{6pt}another:
}}\\
column=0;
\\
{\textbf{for}}\hspace{6pt}k=1:anz
\\
\hspace{24pt}
\\
\hspace{24pt}{\textbf{for}}\hspace{6pt}j=1:rep(k)
\\
\hspace{48pt}
\\
\hspace{48pt}{\it{\%reduceddata:\hspace{6pt}matrix\hspace{6pt}without\hspace{6pt}{'}column{'}th\hspace{6pt}measurement
}}\\
\hspace{48pt}column=column+1;
\\
\hspace{48pt}{\textbf{if}}\hspace{6pt}column==1
\\
\hspace{72pt}reduceddata=data(:,2:n);
\\
\hspace{48pt}{\textbf{elseif}}\hspace{6pt}column==n
\\
\hspace{72pt}reduceddata=data(:,1:n\dash{}1);
\\
\hspace{48pt}{\textbf{else}}
\\
\hspace{72pt}reduceddata={[}data(:,1:column\dash{}1),data(:,column+1:n){]};
\\
\hspace{48pt}{\textbf{end}}
\\
\hspace{48pt}
\\
\hspace{48pt}{\it{\%reducing\hspace{6pt}number\hspace{6pt}of\hspace{6pt}measurements\hspace{6pt}in\hspace{6pt}concerned\hspace{6pt}group:
}}\\
\hspace{48pt}reducedrep=rep;
\\
\hspace{48pt}reducedrep(k)=reducedrep(k)\dash{}1;\\
\\
\hspace{48pt}{\it{\%DPCA:
}}\\
\hspace{48pt}{[}dloading,dscore,dvariance,dintvar{]}=dpca(reduceddata,anz,reducedrep);
\\
\hspace{48pt}
\\
\hspace{48pt}{\it{\%scores\hspace{6pt}plot:
}}\\
\hspace{48pt}plotdpc2dmitellipse(dscore,dvariance,anz,reducedrep,2);
\\
\hspace{48pt}
\\
\hspace{48pt}{\it{\%projection\hspace{6pt}of\hspace{6pt}the\hspace{6pt}left\hspace{6pt}out\hspace{6pt}measurement:
}}\\
\hspace{48pt}dpcaprojektion(dloading,dintvar,data(:,column),1,{\texttt{{'}ko{'}}});
\\
\hspace{42pt}\\
\hspace{48pt}{\it{\%halting\hspace{6pt}program\hspace{6pt}before\hspace{6pt}the\hspace{6pt}next\hspace{6pt}measurement\hspace{6pt}is\hspace{6pt}left\hspace{6pt}out:
}}\\
\hspace{48pt}fprintf(1,{\texttt{{'}Press\hspace{6pt}any\hspace{6pt}key\hspace{6pt}to\hspace{6pt}continue!\hspace{6pt}$\backslash$n{'}}})
\\
\hspace{48pt}pause
\\
\hspace{48pt}
\\
\hspace{24pt}{\textbf{end}}
\\
{\textbf{end}}
\\

\\
\hspace{96pt}
\\
\hspace{48pt}
\end{tabbing}}}


==> loo3.tex <==
{{\def\dash{\raise2.1pt\hbox{\rule{5pt}{0.3pt}}\hspace{1pt}}\begin{tabbing}
{\textbf{function}}\hspace{6pt}assignment=loo3(data,anz,rep,dimmax)
\\
{\it{\%assignment=loo(data,anz,rep,dimmax)}}\\
{\it{\%performs\hspace{6pt}DPCA,\hspace{6pt}leaves\hspace{6pt}each\hspace{6pt}measurement\hspace{6pt}out\hspace{6pt}once}}\\
{\it{\%and\hspace{6pt}calculates\hspace{6pt}its\hspace{6pt}scores\hspace{6pt}to\hspace{6pt}assign\hspace{6pt}it\hspace{6pt}to\hspace{6pt}the\hspace{6pt}closest\hspace{6pt}group.}}\\
{\it{\%Closeness\hspace{6pt}is\hspace{6pt}defined\hspace{6pt}by\hspace{6pt}the\hspace{6pt}euclidean\hspace{6pt}distances\hspace{6pt}to\hspace{6pt}the}}\\
{\it{\%center\hspace{6pt}of\hspace{6pt}gravity\hspace{6pt}of\hspace{6pt}a\hspace{6pt}groups\hspace{6pt}data\hspace{6pt}points.}}\\
{\it{\%data:\hspace{6pt}(mxn)\hspace{6pt}matrix:\hspace{6pt}values\hspace{6pt}of\hspace{6pt}m\hspace{6pt}variables\hspace{6pt}in\hspace{6pt}n\hspace{6pt}measurements}}\\
{\it{\%anz:\hspace{6pt}number\hspace{6pt}of\hspace{6pt}groups}}\\
{\it{\%rep:\hspace{6pt}(anz)\dash{}vector:\hspace{6pt}number\hspace{6pt}of\hspace{6pt}measurements\hspace{6pt}per\hspace{6pt}group}}\\
{\it{\%dimmax:\hspace{6pt}highest\hspace{6pt}considered\hspace{6pt}DPC}}\\
{\it{\%assignment:\hspace{6pt}(nx(anz+1))\dash{}matrix:\hspace{6pt}first\hspace{6pt}column:\hspace{6pt}number\hspace{6pt}of\hspace{6pt}the\hspace{6pt}}}\\
{\it{\%\hspace{66pt}closest\hspace{6pt}group\hspace{6pt}to\hspace{6pt}a\hspace{6pt}measurement;\hspace{6pt}2.,3.,...\hspace{6pt}column:\hspace{6pt}}}\\
{\it{\%\hspace{66pt}relative\hspace{6pt}distance\hspace{6pt}to\hspace{6pt}the\hspace{6pt}1.,2.,...\hspace{6pt}group
}}\\

\\
{[}m,n{]}=size(data);
\\

\\
{[}sizerepx,sizerepy{]}=size(rep);
\\
{\textbf{if}}\hspace{6pt}sizerepy==1
\\
\hspace{24pt}rep=repmat(rep,1,anz);
\\
{\textbf{end}}
\\

\\
{\it{\%loop\hspace{6pt}to\hspace{6pt}leave\hspace{6pt}out\hspace{6pt}one\hspace{6pt}measurement\hspace{6pt}after\hspace{6pt}another:
}}\\
column=0;
\\
{\textbf{for}}\hspace{6pt}k=1:anz
\\
\hspace{24pt}
\\
\hspace{24pt}{\textbf{for}}\hspace{6pt}j=1:rep(k)
\\
\hspace{48pt}
\\
\hspace{48pt}{\it{\%reduceddata:\hspace{6pt}matrix\hspace{6pt}without\hspace{6pt}{'}column{'}th\hspace{6pt}measurement:
}}\\
\hspace{48pt}column=column+1;
\\
\hspace{48pt}{\textbf{if}}\hspace{6pt}column==1
\\
\hspace{72pt}reduceddata=data(:,2:n);
\\
\hspace{48pt}{\textbf{elseif}}\hspace{6pt}column==n
\\
\hspace{72pt}reduceddata=data(:,1:n\dash{}1);
\\
\hspace{48pt}{\textbf{else}}
\\
\hspace{72pt}reduceddata={[}data(:,1:column\dash{}1),data(:,column+1:n){]};
\\
\hspace{48pt}{\textbf{end}}
\\
\hspace{48pt}
\\
\hspace{48pt}{\it{\%reducing\hspace{6pt}number\hspace{6pt}of\hspace{6pt}measurements\hspace{6pt}in\hspace{6pt}concerned\hspace{6pt}group:
}}\\
\hspace{48pt}reducedrep=rep;
\\
\hspace{48pt}reducedrep(k)=reducedrep(k)\dash{}1;\\
\\
\hspace{48pt}{\it{\%DPCA:
}}\\
\hspace{48pt}{[}dloading,dscore,dvariance,dintvar{]}=dpca(reduceddata,anz,reducedrep);
\\
\hspace{48pt}
\\
\hspace{48pt}{\it{\%projection\hspace{6pt}of\hspace{6pt}left\hspace{6pt}out\hspace{6pt}measurement:
}}\\
\hspace{48pt}score=dpcaprojektion(dloading,dintvar,data(:,column),1,{\texttt{{'}no{'}}});
\\
\hspace{48pt}\\
\hspace{48pt}{\it{\%loop\hspace{6pt}to\hspace{6pt}calculate\hspace{6pt}distances\hspace{6pt}to\hspace{6pt}all\hspace{6pt}groupmeans:\hspace{48pt}
}}\\
\hspace{48pt}min=1;
\\
\hspace{48pt}max=0;
\\
\hspace{48pt}{\textbf{for}}\hspace{6pt}i=1:anz\\
\hspace{72pt}{\it{\%calculate\hspace{6pt}center\hspace{6pt}of\hspace{6pt}gravity:
}}\\
\hspace{72pt}max=max+reducedrep(i);
\\
\hspace{72pt}dpcmean=mean(dscore(1:dimmax,min:max),2);\\
\hspace{72pt}{\it{\%calculate\hspace{6pt}euclidean\hspace{6pt}distance:
}}\\
\hspace{72pt}distance(i)=0;
\\
\hspace{72pt}{\textbf{for}}\hspace{6pt}h=1:dimmax
\\
\hspace{96pt}distance(i)=distance(i)+(score(h)\dash{}dpcmean(h))\^{}2;
\\
\hspace{72pt}{\textbf{end}}
\\
\hspace{72pt}distance(i)=sqrt(distance(i));
\\
\hspace{72pt}min=min+reducedrep(i);
\\
\hspace{48pt}{\textbf{end}}\\

\\
\hspace{48pt}{\it{\%assign\hspace{6pt}measurement\hspace{6pt}to\hspace{6pt}closest\hspace{6pt}group:
}}\\
\hspace{48pt}{[}minimum,minimumindex{]}=min(distance);
\\
\hspace{48pt}assignment(column,1)=minimumindex;\\

\\
\hspace{48pt}{\it{\%calculate\hspace{6pt}relative\hspace{6pt}distances:
}}\\
\hspace{48pt}{\textbf{for}}\hspace{6pt}i=1:anz
\\
\hspace{72pt}assignment(column,1+i)=distance(i)/minimum;
\\
\hspace{48pt}{\textbf{end}}\hspace{48pt}
\\
\hspace{24pt}{\textbf{end}}
\\
{\textbf{end}}\hspace{36pt}
\end{tabbing}}}


==> matrix.tex <==
{{\def\dash{\raise2.1pt\hbox{\rule{5pt}{0.3pt}}\hspace{1pt}}\begin{tabbing}
{\textbf{function}}\hspace{6pt}X\hspace{6pt}=\hspace{6pt}matrix(X,in)
\\
{\it{\%X\hspace{6pt}=\hspace{6pt}matrix(X,in)}}\\
{\it{\%adds\hspace{6pt}a\hspace{6pt}new\hspace{6pt}measurement\hspace{6pt}to\hspace{6pt}a\hspace{6pt}data\hspace{6pt}matrix}}\\
{\it{\%X:\hspace{6pt}(mxn)\dash{}matrix:\hspace{6pt}values\hspace{6pt}of\hspace{6pt}m\hspace{6pt}variables\hspace{6pt}in\hspace{6pt}n\hspace{6pt}measurements}}\\
{\it{\%in:\hspace{6pt}WinCadence\hspace{6pt}output:\hspace{6pt}unit\hspace{6pt}mass\hspace{6pt}mass\dash{}spectrum}}\\

\\
{[}m,n{]}=size(X);\\
\\
{\it{\%extracting\hspace{6pt}the\hspace{6pt}counts\hspace{6pt}from\hspace{6pt}WinCadence\hspace{6pt}output:
}}\\
in=voll(in,m);\\
\\
{\it{\%appending\hspace{6pt}the\hspace{6pt}new\hspace{6pt}data:
}}\\
X(:,n+1)=in(:,1);
\end{tabbing}}}


==> pca.tex <==
{{\def\dash{\raise2.1pt\hbox{\rule{5pt}{0.3pt}}\hspace{1pt}}\begin{tabbing}
{\textbf{function}}\hspace{6pt}{[}PC,\hspace{6pt}SCORE,\hspace{6pt}V,\hspace{6pt}mn{]}=pca(X);\\
{\it{\%{[}PC,\hspace{6pt}SCORE,\hspace{6pt}V,\hspace{6pt}mn{]}=pca(X)}}\\
{\it{\%performs\hspace{6pt}principal\hspace{6pt}component\hspace{6pt}analysis}}\\
{\it{\%X:\hspace{6pt}(mxn)\dash{}matrix:\hspace{6pt}values\hspace{6pt}of\hspace{6pt}m\hspace{6pt}variables\hspace{6pt}for\hspace{6pt}n\hspace{6pt}measurements}}\\
{\it{\%PC:\hspace{6pt}(mxm)\dash{}matrix:\hspace{6pt}loadings\hspace{6pt}of\hspace{6pt}m\hspace{6pt}PC\hspace{6pt}as\hspace{6pt}m\hspace{6pt}columns}}\\
{\it{\%SCORE:\hspace{6pt}(mxn)\dash{}matrix:\hspace{6pt}scores\hspace{6pt}of\hspace{6pt}m\hspace{6pt}PC\hspace{6pt}for\hspace{6pt}n\hspace{6pt}measurements}}\\
{\it{\%V:\hspace{6pt}(m)\dash{}vector:\hspace{6pt}variance\hspace{6pt}captured\hspace{6pt}by\hspace{6pt}the\hspace{6pt}m\hspace{6pt}PC}}\\
{\it{\%mn:\hspace{6pt}(m)\dash{}vector:\hspace{6pt}mean\hspace{6pt}values\hspace{6pt}of\hspace{6pt}the\hspace{6pt}m\hspace{6pt}variables}}\\
{\it{\%for\hspace{6pt}details\hspace{6pt}on\hspace{6pt}the\hspace{6pt}PCA\hspace{6pt}algorithm\hspace{6pt}see\hspace{6pt}J.\hspace{6pt}Shlens,\hspace{6pt}}}\\
{\it{\%A\hspace{6pt}tutorial\hspace{6pt}on\hspace{6pt}principal\hspace{6pt}component\hspace{6pt}analysis,\hspace{6pt}10/12/2005}}\\
\\
{[}m,n{]}=size(X);\\
\\
{\it{\%scaling\hspace{6pt}by\hspace{6pt}total\hspace{6pt}intensity:}}\\
{\textbf{for}}\hspace{6pt}k=1:n\\
\hspace{24pt}X(:,k)=X(:,k)/sum(X(:,k));\\
{\textbf{end}}\\
\\
{\it{\%mean\dash{}centering:}}\\
mn=mean(X,2);\\
X=X\dash{}repmat(mn,1,n);\\
\\
{\it{\%auxiliary\hspace{6pt}matrix\hspace{6pt}for\hspace{6pt}SVD:}}\\
Y=X{'}/sqrt(n\dash{}1);\\
\\
{\it{\%singular\hspace{6pt}value\hspace{6pt}decomposition:}}\\
{[}u,S,PC{]}=svd(Y);\\
\\
{\it{\%variances\hspace{6pt}\dash{}$>$\hspace{6pt}m\dash{}vector\hspace{6pt}V:}}\\
S=diag(S);\\
V=S.$\ast$S;\\
\\
{\it{\%projection\hspace{6pt}\dash{}$>$\hspace{6pt}(mxn)\dash{}matrix\hspace{6pt}SCORE:}}\\
SCORE=PC{'}$\ast$X;\\
\\
{\it{\%saving\hspace{6pt}loadings\hspace{6pt}and\hspace{6pt}scores:}}\\
save\hspace{6pt}ploading.dat\hspace{6pt}PC\hspace{6pt}\dash{}ascii;\\
save\hspace{6pt}pscore.dat\hspace{6pt}SCORE\hspace{6pt}\dash{}ascii;
\end{tabbing}}}


==> pcaprojektion.tex <==
{{\def\dash{\raise2.1pt\hbox{\rule{5pt}{0.3pt}}\hspace{1pt}}\begin{tabbing}
{\textbf{function}}\hspace{6pt}score=pcaprojektion(loading,mitte,data,index,stil)\\
{\it{\%dpcaprojektion(loading,mitte,data,index,stil)}}\\
{\it{\%projects\hspace{6pt}a\hspace{6pt}data\hspace{6pt}matrix\hspace{6pt}using\hspace{6pt}PC\hspace{6pt}loadings\hspace{6pt}into\hspace{6pt}a\hspace{6pt}scores\hspace{6pt}plot}}\\
{\it{\%loading:\hspace{6pt}(mxm)\dash{}matrix:\hspace{6pt}loadings\hspace{6pt}of\hspace{6pt}m\hspace{6pt}PC\hspace{6pt}as\hspace{6pt}m\hspace{6pt}columns}}\\
{\it{\%mitte:\hspace{6pt}m\dash{}vector:\hspace{6pt}mean\hspace{6pt}values\hspace{6pt}of\hspace{6pt}m\hspace{6pt}variables\hspace{6pt}for\hspace{6pt}the\hspace{6pt}original\hspace{6pt}data}}\\
{\it{\%data:\hspace{6pt}(mxn)\dash{}matrix:\hspace{6pt}values\hspace{6pt}of\hspace{6pt}m\hspace{6pt}variables\hspace{6pt}for\hspace{6pt}n\hspace{6pt}new\hspace{6pt}measurements}}\\
{\it{\%index:\hspace{6pt}number\hspace{6pt}of\hspace{6pt}first\hspace{6pt}displayed\hspace{6pt}PC\hspace{6pt}in\hspace{6pt}the\hspace{6pt}scores\hspace{6pt}plot}}\\
{\it{\%stil:\hspace{6pt}style\hspace{6pt}of\hspace{6pt}the\hspace{6pt}projected\hspace{6pt}data\hspace{6pt}points}}\\
{\it{\%score:\hspace{6pt}(mxn)\dash{}matrix:\hspace{6pt}projected\hspace{6pt}scores\hspace{6pt}of\hspace{6pt}m\hspace{6pt}PC\hspace{6pt}for\hspace{6pt}n\hspace{6pt}new\hspace{6pt}measurements
}}\\

\\
{[}m,n{]}=size(data);
\\

\\
{\it{\%scaling\hspace{6pt}of\hspace{6pt}measurements\hspace{6pt}by\hspace{6pt}total\hspace{6pt}intensity:
}}\\
{\textbf{for}}\hspace{6pt}k=1:n
\\
\hspace{24pt}data(:,k)=data(:,k)/sum(data(:,k));
\\
{\textbf{end}}
\\
\\
{\it{\%mean\hspace{6pt}centering:
}}\\
centered=data\dash{}repmat(mitte,1,n);\\
\\
{\it{\%projection:
}}\\
score=loading{'}$\ast$centered;
\\
\\
{\it{\%plotting\hspace{6pt}can\hspace{6pt}be\hspace{6pt}prevented\hspace{6pt}with\hspace{6pt}style\hspace{6pt}{'}no{'}:
}}\\
{\textbf{if}}\hspace{6pt}stil=={\texttt{{'}no{'}}}
\\
\hspace{24pt}{\textbf{return}}
\\
{\textbf{end}}
\\
\\
{\it{\%plotting:
}}\\
hold\hspace{6pt}on
\\
plot(score(index,:),score(index+1,:),stil);
\end{tabbing}}}


==> plotdpc2d.tex <==
{{\def\dash{\raise2.1pt\hbox{\rule{5pt}{0.3pt}}\hspace{1pt}}\begin{tabbing}
{\textbf{function}}\hspace{6pt}plotdpc2d(PC,SCORE,relvariance,anz,rep,omax)
\\
{\it{\%plotdpc2d(PC,SCORE,relvariance,anz,rep,omax)}}\\
{\it{\%creates\hspace{6pt}2D\hspace{6pt}scores\hspace{6pt}and\hspace{6pt}loadings\hspace{6pt}plots\hspace{6pt}}}\\
{\it{\%PC:\hspace{6pt}(mxm)\dash{}matrix:\hspace{6pt}loadings\hspace{6pt}of\hspace{6pt}m\hspace{6pt}DPC\hspace{6pt}as\hspace{6pt}m\hspace{6pt}columns}}\\
{\it{\%SCORE:\hspace{6pt}(mxn)\dash{}matrix:\hspace{6pt}scores\hspace{6pt}of\hspace{6pt}m\hspace{6pt}DPC\hspace{6pt}for\hspace{6pt}n\hspace{6pt}measurements}}\\
{\it{\%relvariance:\hspace{6pt}(m)\dash{}vector:\hspace{6pt}relative\hspace{6pt}variance\hspace{6pt}captured\hspace{6pt}by\hspace{6pt}the\hspace{6pt}m\hspace{6pt}DPC}}\\
{\it{\%anz:\hspace{6pt}number\hspace{6pt}of\hspace{6pt}groups}}\\
{\it{\%rep:\hspace{6pt}(anz)\dash{}vector:\hspace{6pt}number\hspace{6pt}of\hspace{6pt}measurements\hspace{6pt}per\hspace{6pt}group}}\\
{\it{\%omax:\hspace{6pt}highest\hspace{6pt}dimension\hspace{6pt}plotted\hspace{6pt}
}}\\

\\
{\textbf{if}}\hspace{6pt}omax$<$2
\\
\hspace{24pt}fprintf(1,{\texttt{{'}Error:\hspace{6pt}Maximum\hspace{6pt}principal\hspace{6pt}component\hspace{6pt}must\hspace{6pt}be\hspace{6pt}greater\hspace{6pt}one!{'}}})
\\
\hspace{24pt}{\textbf{return}}
\\
{\textbf{end}}
\\
\\
{\it{\%scaling\hspace{6pt}variances:
}}\\
{\textbf{if}}\hspace{6pt}sum(relvariance)\~{}=100
\\
\hspace{24pt}relvariance=relvariance/sum(relvariance)$\ast$100;
\\
{\textbf{end}}
\\

\\
{[}sizerepx,sizerepy{]}=size(rep);
\\
{\textbf{if}}\hspace{6pt}sizerepy==1
\\
\hspace{24pt}rep=repmat(rep,1,anz);
\\
{\textbf{end}}
\\
\\
{\it{\%loop\hspace{6pt}to\hspace{6pt}create\hspace{6pt}more\hspace{6pt}than\hspace{6pt}one\hspace{6pt}plot:
}}\\
{\textbf{for}}\hspace{6pt}o=2:omax
\\

\\
figure
\\
\\
{\it{\%loadings\hspace{6pt}plot:
}}\\
subplot(2,1,1)
\\
plot(PC(:,o\dash{}1),PC(:,o),{\texttt{{'}kx{'}}});
\\
grid\hspace{6pt}on
\\
title({\texttt{{'}Loadings\hspace{6pt}Plot{'}}});
\\
xlabel({[}{\texttt{{'}DPC\hspace{6pt}{'}}}\hspace{6pt}int2str(o\dash{}1){]});
\\
ylabel({[}{\texttt{{'}DPC\hspace{6pt}{'}}}\hspace{6pt}int2str(o){]});
\\
\\
{\it{\%scores\hspace{6pt}plot\hspace{6pt}with\hspace{6pt}different\hspace{6pt}styles\hspace{6pt}for\hspace{6pt}different\hspace{6pt}groups:
}}\\
subplot(2,1,2)
\\
hold\hspace{6pt}on\\
\\
{\it{\%loop\hspace{6pt}for\hspace{6pt}different\hspace{6pt}groups:
}}\\
min=1;
\\
max=0;
\\
{\textbf{for}}\hspace{6pt}k=1:anz
\\
\hspace{24pt}max=max+rep(k);
\\
\hspace{24pt}{\textbf{switch}}\hspace{6pt}k
\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}1
\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}ro{'}}});
\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}2
\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}bx{'}}});
\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}3
\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}g+{'}}});
\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}4
\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}c$\ast${'}}});
\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}5
\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}ms{'}}});
\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}6
\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}yd{'}}});
\\
\hspace{48pt}{\textbf{otherwise}}
\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}k\^{}{'}}});
\\
\hspace{66pt}fprintf(1,{\texttt{{'}Cannot\hspace{6pt}plot\hspace{6pt}more\hspace{6pt}than\hspace{6pt}six\hspace{6pt}groups!{'}}});
\\
\hspace{24pt}{\textbf{end}}
\\
\hspace{24pt}min=min+rep(k);
\\
{\textbf{end}}
\\
grid\hspace{6pt}on
\\
title({\texttt{{'}Scores\hspace{6pt}Plot{'}}});
\\
xlabel({[}{\texttt{{'}DPC\hspace{6pt}{'}}}\hspace{6pt}int2str(o\dash{}1)\hspace{6pt}{\texttt{{'}\hspace{6pt}({'}}}\hspace{6pt}int2str(relvariance(o\dash{}1))\hspace{6pt}{\texttt{{'}\%){'}}}{]});
\\
ylabel({[}{\texttt{{'}DPC\hspace{6pt}{'}}}\hspace{6pt}int2str(o)\hspace{6pt}{\texttt{{'}\hspace{6pt}({'}}}\hspace{6pt}int2str(relvariance(o))\hspace{6pt}{\texttt{{'}\%){'}}}{]});
\\

\\
{\textbf{end}}
\end{tabbing}}}


==> plotdpc2dmitellipse.tex <==
{{\def\dash{\raise2.1pt\hbox{\rule{5pt}{0.3pt}}\hspace{1pt}}\begin{tabbing}
{\textbf{function}}\hspace{6pt}plotdpc2dmitellipse(SCORE,relvariance,anz,rep,omax)\\
{\it{\%plotdpc2dmitellipse(SCORE,relvariance,anz,rep,omax)}}\\
{\it{\%creates\hspace{6pt}2D\hspace{6pt}scores\hspace{6pt}plots\hspace{6pt}with\hspace{6pt}probability\hspace{6pt}ellipses}}\\
{\it{\%SCORE:\hspace{6pt}(mxn)\dash{}matrix:\hspace{6pt}scores\hspace{6pt}of\hspace{6pt}m\hspace{6pt}DPC\hspace{6pt}for\hspace{6pt}n\hspace{6pt}measurements}}\\
{\it{\%relvariance:\hspace{6pt}(m)\dash{}vector:\hspace{6pt}relative\hspace{6pt}variance\hspace{6pt}captured\hspace{6pt}by\hspace{6pt}the\hspace{6pt}m\hspace{6pt}DPC}}\\
{\it{\%anz:\hspace{6pt}number\hspace{6pt}of\hspace{6pt}groups}}\\
{\it{\%rep:\hspace{6pt}(anz)\dash{}vector:\hspace{6pt}number\hspace{6pt}of\hspace{6pt}measurements\hspace{6pt}per\hspace{6pt}group}}\\
{\it{\%omax:\hspace{6pt}highest\hspace{6pt}dimension\hspace{6pt}plotted\hspace{6pt}}}\\
\\
{\textbf{if}}\hspace{6pt}omax$<$2\\
\hspace{24pt}fprintf(1,{\texttt{{'}Error:\hspace{6pt}Maximum\hspace{6pt}principal\hspace{6pt}component\hspace{6pt}must\hspace{6pt}be\hspace{6pt}greater\hspace{6pt}one!{'}}})\\
\hspace{24pt}{\textbf{return}}\\
{\textbf{end}}\\
\\
{\it{\%scaling\hspace{6pt}variances:}}\\
{\textbf{if}}\hspace{6pt}sum(relvariance)\~{}=100\\
\hspace{24pt}relvariance=relvariance/sum(relvariance)$\ast$100;\\
{\textbf{end}}\\
\\
{[}sizerepx,sizerepy{]}=size(rep);\\
{\textbf{if}}\hspace{6pt}sizerepy==1\\
\hspace{24pt}rep=repmat(rep,1,anz);\\
{\textbf{end}}\\
\\
{\it{\%loop\hspace{6pt}to\hspace{6pt}create\hspace{6pt}more\hspace{6pt}than\hspace{6pt}one\hspace{6pt}plot:}}\\
{\textbf{for}}\hspace{6pt}o=2:omax\\
\\
figure\\
\\
{\it{\%scores\hspace{6pt}plot\hspace{6pt}with\hspace{6pt}different\hspace{6pt}styles\hspace{6pt}for\hspace{6pt}different\hspace{6pt}groups:}}\\
hold\hspace{6pt}on\\
min=1;\\
max=0;\\
\\
{\it{\%loop\hspace{6pt}for\hspace{6pt}different\hspace{6pt}groups:}}\\
{\textbf{for}}\hspace{6pt}k=1:anz\\
\\
\hspace{24pt}{\it{\%critical\hspace{6pt}value\hspace{6pt}of\hspace{6pt}F\dash{}distribution\hspace{6pt}for\hspace{6pt}2\hspace{6pt}variables,}}\\
\hspace{24pt}{\it{\%rep(k)\hspace{6pt}measurements\hspace{6pt}and\hspace{6pt}95\%\hspace{6pt}confidence\hspace{6pt}limit:}}\\
\hspace{24pt}F=Fdistribution(rep(k));\\
\\
\hspace{24pt}{\it{\%calculate\hspace{6pt}critical\hspace{6pt}TSquare\hspace{6pt}value\hspace{6pt}for\hspace{6pt}the\hspace{6pt}ellipses:}}\\
\hspace{24pt}Tsquare=2$\ast$(rep(k)\dash{}1)/(rep(k)\dash{}2)$\ast$F;\\
\\
\hspace{24pt}max=max+rep(k);\\
\hspace{24pt}{\textbf{switch}}\hspace{6pt}k\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}1\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}ro{'}}});\\
\hspace{72pt}ellipse(SCORE(o\dash{}1:o,min:max),Tsquare,{\texttt{{'}r{'}}});\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}2\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}bx{'}}});\\
\hspace{72pt}ellipse(SCORE(o\dash{}1:o,min:max),Tsquare,{\texttt{{'}b{'}}});\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}3\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}g+{'}}});\\
\hspace{72pt}ellipse(SCORE(o\dash{}1:o,min:max),Tsquare,{\texttt{{'}g{'}}});\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}4\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}c$\ast${'}}});\\
\hspace{72pt}ellipse(SCORE(o\dash{}1:o,min:max),Tsquare,{\texttt{{'}c{'}}});\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}5\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}ms{'}}});\\
\hspace{72pt}ellipse(SCORE(o\dash{}1:o,min:max),Tsquare,{\texttt{{'}m{'}}});\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}6\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}yd{'}}});\\
\hspace{72pt}ellipse(SCORE(o\dash{}1:o,min:max),Tsquare,{\texttt{{'}y{'}}});\\
\hspace{48pt}{\textbf{otherwise}}\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}k\^{}{'}}});\\
\hspace{72pt}fprintf(1,{\texttt{{'}Cannot\hspace{6pt}plot\hspace{6pt}more\hspace{6pt}than\hspace{6pt}six\hspace{6pt}groups!{'}}});\\
\hspace{24pt}{\textbf{end}}\\
\hspace{24pt}min=min+rep(k);\\
{\textbf{end}}\\
grid\hspace{6pt}on\\
title({\texttt{{'}Scores\hspace{6pt}Plot{'}}});\\
xlabel({[}{\texttt{{'}DPC\hspace{6pt}{'}}}\hspace{6pt}int2str(o\dash{}1)\hspace{6pt}{\texttt{{'}\hspace{6pt}({'}}}\hspace{6pt}int2str(relvariance(o\dash{}1))\hspace{6pt}{\texttt{{'}\%){'}}}{]});\\
ylabel({[}{\texttt{{'}DPC\hspace{6pt}{'}}}\hspace{6pt}int2str(o)\hspace{6pt}{\texttt{{'}\hspace{6pt}({'}}}\hspace{6pt}int2str(relvariance(o))\hspace{6pt}{\texttt{{'}\%){'}}}{]});\\
\\
{\textbf{end}}
\end{tabbing}}}


==> plotdpc2dmitellipse2.tex <==
{{\def\dash{\raise2.1pt\hbox{\rule{5pt}{0.3pt}}\hspace{1pt}}\begin{tabbing}
{\textbf{function}}\hspace{6pt}plotdpc2dmitellipse2(PC,SCORE,relvariance,anz,rep,omax)\\
{\it{\%plotdpc2dmitellipse2(PC,SCORE,relvariance,anz,rep,omax)}}\\
{\it{\%creates\hspace{6pt}2D\hspace{6pt}scores\hspace{6pt}plots\hspace{6pt}with\hspace{6pt}probability\hspace{6pt}ellipses\hspace{6pt}and\hspace{6pt}loadings\hspace{6pt}plots\hspace{6pt}}}\\
{\it{\%PC:\hspace{6pt}(mxm)\dash{}matrix:\hspace{6pt}loadings\hspace{6pt}of\hspace{6pt}m\hspace{6pt}DPC\hspace{6pt}as\hspace{6pt}m\hspace{6pt}columns}}\\
{\it{\%SCORE:\hspace{6pt}(mxn)\dash{}matrix:\hspace{6pt}scores\hspace{6pt}of\hspace{6pt}m\hspace{6pt}DPC\hspace{6pt}for\hspace{6pt}n\hspace{6pt}measurements}}\\
{\it{\%relvariance:\hspace{6pt}(m)\dash{}vector:\hspace{6pt}relative\hspace{6pt}variance\hspace{6pt}captured\hspace{6pt}by\hspace{6pt}the\hspace{6pt}m\hspace{6pt}DPC}}\\
{\it{\%anz:\hspace{6pt}number\hspace{6pt}of\hspace{6pt}groups}}\\
{\it{\%rep:\hspace{6pt}(anz)\dash{}vector:\hspace{6pt}number\hspace{6pt}of\hspace{6pt}measurements\hspace{6pt}per\hspace{6pt}group}}\\
{\it{\%omax:\hspace{6pt}highest\hspace{6pt}dimension\hspace{6pt}plotted\hspace{6pt}}}\\
\\
{\textbf{if}}\hspace{6pt}omax$<$2\\
\hspace{24pt}fprintf(1,{\texttt{{'}Error:\hspace{6pt}Maximum\hspace{6pt}principal\hspace{6pt}component\hspace{6pt}must\hspace{6pt}be\hspace{6pt}greater\hspace{6pt}one!{'}}})\\
\hspace{24pt}{\textbf{return}}\\
{\textbf{end}}\\
\\
{\it{\%scaling\hspace{6pt}variances:}}\\
{\textbf{if}}\hspace{6pt}sum(relvariance)\~{}=100\\
\hspace{24pt}relvariance=relvariance/sum(relvariance)$\ast$100;\\
{\textbf{end}}\\
\\
{[}sizerepx,sizerepy{]}=size(rep);\\
{\textbf{if}}\hspace{6pt}sizerepy==1\\
\hspace{24pt}rep=repmat(rep,1,anz);\\
{\textbf{end}}\\
\\
{\it{\%loop\hspace{6pt}to\hspace{6pt}create\hspace{6pt}more\hspace{6pt}than\hspace{6pt}one\hspace{6pt}plot:}}\\
{\textbf{for}}\hspace{6pt}o=2:omax\\
\\
figure\\
\\
{\it{\%loadings\hspace{6pt}plot:}}\\
subplot(2,1,1)\\
plot(PC(:,o\dash{}1),PC(:,o),{\texttt{{'}kx{'}}});\\
grid\hspace{6pt}on\\
title({\texttt{{'}Loadings\hspace{6pt}Plot{'}}});\\
xlabel({[}{\texttt{{'}DPC\hspace{6pt}{'}}}\hspace{6pt}int2str(o\dash{}1){]});\\
ylabel({[}{\texttt{{'}DPC\hspace{6pt}{'}}}\hspace{6pt}int2str(o){]});\\
\\
{\it{\%scores\hspace{6pt}plot\hspace{6pt}with\hspace{6pt}different\hspace{6pt}styles\hspace{6pt}for\hspace{6pt}different\hspace{6pt}groups:}}\\
subplot(2,1,2)\\
hold\hspace{6pt}on\\
min=1;\\
max=0;\\
\\
{\it{\%loop\hspace{6pt}for\hspace{6pt}different\hspace{6pt}groups:}}\\
{\textbf{for}}\hspace{6pt}k=1:anz\\
\\
\hspace{24pt}{\it{\%critical\hspace{6pt}value\hspace{6pt}of\hspace{6pt}F\dash{}distribution\hspace{6pt}for\hspace{6pt}2\hspace{6pt}variables,}}\\
\hspace{24pt}{\it{\%rep(k)\hspace{6pt}measurements\hspace{6pt}and\hspace{6pt}95\%\hspace{6pt}confidence\hspace{6pt}limit:}}\\
\hspace{24pt}F=Fdistribution(rep(k));\\
\\
\hspace{24pt}{\it{\%calculate\hspace{6pt}critical\hspace{6pt}TSquare\hspace{6pt}value\hspace{6pt}for\hspace{6pt}the\hspace{6pt}ellipses:}}\\
\hspace{24pt}Tsquare=2$\ast$(rep(k)\dash{}1)/(rep(k)\dash{}2)$\ast$F;\\
\\
\hspace{24pt}max=max+rep(k);\\
\hspace{24pt}{\textbf{switch}}\hspace{6pt}k\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}1\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}ro{'}}});\\
\hspace{72pt}ellipse(SCORE(o\dash{}1:o,min:max),Tsquare,{\texttt{{'}r{'}}});\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}2\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}bx{'}}});\\
\hspace{72pt}ellipse(SCORE(o\dash{}1:o,min:max),Tsquare,{\texttt{{'}b{'}}});\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}3\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}g+{'}}});\\
\hspace{72pt}ellipse(SCORE(o\dash{}1:o,min:max),Tsquare,{\texttt{{'}g{'}}});\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}4\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}c$\ast${'}}});\\
\hspace{72pt}ellipse(SCORE(o\dash{}1:o,min:max),Tsquare,{\texttt{{'}c{'}}});\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}5\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}ms{'}}});\\
\hspace{72pt}ellipse(SCORE(o\dash{}1:o,min:max),Tsquare,{\texttt{{'}m{'}}});\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}6\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}yd{'}}});\\
\hspace{72pt}ellipse(SCORE(o\dash{}1:o,min:max),Tsquare,{\texttt{{'}y{'}}});\\
\hspace{48pt}{\textbf{otherwise}}\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}k\^{}{'}}});\\
\hspace{72pt}fprintf(1,{\texttt{{'}Cannot\hspace{6pt}plot\hspace{6pt}more\hspace{6pt}than\hspace{6pt}six\hspace{6pt}groups!{'}}});\\
\hspace{24pt}{\textbf{end}}\\
\hspace{24pt}min=min+rep(k);\\
{\textbf{end}}\\
grid\hspace{6pt}on\\
title({\texttt{{'}Scores\hspace{6pt}Plot{'}}});\\
xlabel({[}{\texttt{{'}DPC\hspace{6pt}{'}}}\hspace{6pt}int2str(o\dash{}1)\hspace{6pt}{\texttt{{'}\hspace{6pt}({'}}}\hspace{6pt}int2str(relvariance(o\dash{}1))\hspace{6pt}{\texttt{{'}\%){'}}}{]});\\
ylabel({[}{\texttt{{'}DPC\hspace{6pt}{'}}}\hspace{6pt}int2str(o)\hspace{6pt}{\texttt{{'}\hspace{6pt}({'}}}\hspace{6pt}int2str(relvariance(o))\hspace{6pt}{\texttt{{'}\%){'}}}{]});\\
\\
{\textbf{end}}
\end{tabbing}}}


==> plotpc2d.tex <==
{{\def\dash{\raise2.1pt\hbox{\rule{5pt}{0.3pt}}\hspace{1pt}}\begin{tabbing}
{\textbf{function}}\hspace{6pt}plotpc2d(PC,SCORE,relvariance,anz,rep,omax)\\
{\it{\%plotpc2d(PC,SCORE,relvariance,anz,rep,omax)}}\\
{\it{\%creates\hspace{6pt}2D\hspace{6pt}scores\hspace{6pt}plots\hspace{6pt}and\hspace{6pt}loadings\hspace{6pt}plots}}\\
{\it{\%PC:\hspace{6pt}(mxm)\dash{}matrix:\hspace{6pt}loadings\hspace{6pt}of\hspace{6pt}m\hspace{6pt}PC\hspace{6pt}as\hspace{6pt}m\hspace{6pt}columns}}\\
{\it{\%SCORE:\hspace{6pt}(mxn)\dash{}matrix:\hspace{6pt}scores\hspace{6pt}of\hspace{6pt}m\hspace{6pt}PC\hspace{6pt}for\hspace{6pt}n\hspace{6pt}measurements}}\\
{\it{\%relvariance:\hspace{6pt}(m)\dash{}vector:\hspace{6pt}relative\hspace{6pt}variance\hspace{6pt}captured\hspace{6pt}by\hspace{6pt}the\hspace{6pt}m\hspace{6pt}PC}}\\
{\it{\%anz:\hspace{6pt}number\hspace{6pt}of\hspace{6pt}groups}}\\
{\it{\%rep:\hspace{6pt}(anz)\dash{}vector:\hspace{6pt}number\hspace{6pt}of\hspace{6pt}measurements\hspace{6pt}per\hspace{6pt}group}}\\
{\it{\%omax:\hspace{6pt}highest\hspace{6pt}dimension\hspace{6pt}plotted\hspace{6pt}}}\\
\\
{\textbf{if}}\hspace{6pt}omax$<$2\\
\hspace{24pt}fprintf(1,{\texttt{{'}Error:\hspace{6pt}Maximum\hspace{6pt}principal\hspace{6pt}component\hspace{6pt}must\hspace{6pt}be\hspace{6pt}grater\hspace{6pt}1!{'}}})\\
\hspace{24pt}{\textbf{return}}\\
{\textbf{end}}\\
\\
{\it{\%scaling\hspace{6pt}variances\hspace{6pt}if\hspace{6pt}necessary:}}\\
{\textbf{if}}\hspace{6pt}sum(relvariance)\~{}=100\\
\hspace{24pt}relvariance=relvariance/sum(relvariance)$\ast$100;\\
{\textbf{end}}\\
\\
{[}sizerepx,sizerepy{]}=size(rep);\\
{\textbf{if}}\hspace{6pt}sizerepy==1\\
\hspace{24pt}rep=repmat(rep,1,anz);\\
{\textbf{end}}\\
\\
{\it{\%loop\hspace{6pt}for\hspace{6pt}different\hspace{6pt}plots:}}\\
{\textbf{for}}\hspace{6pt}o=2:omax\\
\\
figure\\
\\
{\it{\%loadings\hspace{6pt}plot:}}\\
subplot(2,1,1)\\
plot(PC(:,o\dash{}1),PC(:,o),{\texttt{{'}kx{'}}});\\
grid\hspace{6pt}on\\
title({\texttt{{'}Loadings\hspace{6pt}Plot{'}}});\\
xlabel({[}{\texttt{{'}PC\hspace{6pt}{'}}}\hspace{6pt}int2str(o\dash{}1){]});\\
ylabel({[}{\texttt{{'}PC\hspace{6pt}{'}}}\hspace{6pt}int2str(o){]});\\
\\
subplot(2,1,2)\\
\\
{\it{\%scores\hspace{6pt}plots:}}\\
hold\hspace{6pt}on\\
min=1;\\
max=0;\\
\\
{\it{\%loop\hspace{6pt}for\hspace{6pt}different\hspace{6pt}groups:}}\\
{\textbf{for}}\hspace{6pt}k=1:anz\\
\hspace{24pt}max=max+rep(k);\\
\hspace{24pt}{\textbf{switch}}\hspace{6pt}k\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}1\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}ro{'}}});\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}2\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}bx{'}}});\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}3\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}g+{'}}});\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}4\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}c$\ast${'}}});\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}5\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}ms{'}}});;\\
\hspace{48pt}{\textbf{case}}\hspace{6pt}6\\
\hspace{72pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}yd{'}}});\\
\hspace{48pt}{\textbf{otherwise}}\\
\hspace{66pt}plot(SCORE(o\dash{}1,min:max),SCORE(o,min:max),{\texttt{{'}k\^{}{'}}});\\
\hspace{66pt}fprintf(1,{\texttt{{'}Cannot\hspace{6pt}plot\hspace{6pt}more\hspace{6pt}than\hspace{6pt}6\hspace{6pt}groups!{'}}});\\
\hspace{24pt}{\textbf{end}}\\
\hspace{24pt}min=min+rep(k);\\
{\textbf{end}}\\
grid\hspace{6pt}on\\
title({\texttt{{'}Scores\hspace{6pt}Plot{'}}});\\
xlabel({[}{\texttt{{'}PC\hspace{6pt}{'}}}\hspace{6pt}int2str(o\dash{}1)\hspace{6pt}{\texttt{{'}\hspace{6pt}({'}}}\hspace{6pt}int2str(relvariance(o\dash{}1))\hspace{6pt}{\texttt{{'}\%){'}}}{]});\\
ylabel({[}{\texttt{{'}PC\hspace{6pt}{'}}}\hspace{6pt}int2str(o)\hspace{6pt}{\texttt{{'}\hspace{6pt}({'}}}\hspace{6pt}int2str(relvariance(o))\hspace{6pt}{\texttt{{'}\%){'}}}{]});\\
\\
{\textbf{end}}
\end{tabbing}}}


==> silanweg.tex <==
{{\def\dash{\raise2.1pt\hbox{\rule{5pt}{0.3pt}}\hspace{1pt}}\begin{tabbing}
{\textbf{function}}\hspace{6pt}output=silanweg(input,background);\\
{\it{\%output=silanweg(input,background);}}\\
{\it{\%substracts\hspace{6pt}a\hspace{6pt}background\hspace{6pt}spectrum\hspace{6pt}from\hspace{6pt}mass\hspace{6pt}spectra;}}\\
{\it{\%the\hspace{6pt}background\hspace{6pt}is\hspace{6pt}scaled\hspace{6pt}to\hspace{6pt}have\hspace{6pt}the\hspace{6pt}same\hspace{6pt}value\hspace{6pt}as}}\\
{\it{\%the\hspace{6pt}measurement\hspace{6pt}at\hspace{6pt}the\hspace{6pt}28th\hspace{6pt}variable\hspace{6pt}}}\\
{\it{\%input:\hspace{6pt}(mxn)\dash{}matrix:\hspace{6pt}values\hspace{6pt}of\hspace{6pt}m\hspace{6pt}variables\hspace{6pt}in\hspace{6pt}n\hspace{6pt}spectra}}\\
{\it{\%background:\hspace{6pt}(mx1)\dash{}vector:\hspace{6pt}background\hspace{6pt}values\hspace{6pt}of\hspace{6pt}m\hspace{6pt}variables\hspace{6pt}}}\\
\\
{[}m,n{]}=size(input);\\
{[}mm,nn{]}=size(background);\\
\\
{\textbf{if}}\hspace{6pt}mm\~{}=m\\
\hspace{24pt}fprintf(1,{\texttt{{'}Error:\hspace{6pt}Measurements\hspace{6pt}and\hspace{6pt}background}} \\
{\texttt{\must\hspace{6pt}have\hspace{6pt}the\hspace{6pt}same\hspace{6pt}number\hspace{6pt}of\hspace{6pt}rows!{'}}})\\
\hspace{24pt}{\textbf{return}}\\
{\textbf{end}}\\
\\
{\it{\%loop\hspace{6pt}to\hspace{6pt}treat\hspace{6pt}different\hspace{6pt}measurements:}}\\
{\textbf{for}}\hspace{6pt}k=1:n\\
\hspace{24pt}factor=input(28,k)/background(28,1);\\
\hspace{24pt}output(:,k)=input(:,k)\dash{}factor$\ast$background(:,1);\\
{\textbf{end}}
\end{tabbing}}}


==> voll.tex <==
{{\def\dash{\raise2.1pt\hbox{\rule{5pt}{0.3pt}}\hspace{1pt}}\begin{tabbing}
{\textbf{function}}\hspace{6pt}filled\hspace{6pt}=\hspace{6pt}voll(in,m);
\\
{\it{\%filled\hspace{6pt}=\hspace{6pt}voll(in,m)}}\\
{\it{\%extracts\hspace{6pt}counts\hspace{6pt}from\hspace{6pt}a\hspace{6pt}WinCadence\hspace{6pt}output\hspace{6pt}unit\hspace{6pt}mass}}\\
{\it{\%mass\hspace{6pt}spectrum}}\\
{\it{\%in:\hspace{6pt}(?x3)\dash{}matrix:\hspace{6pt}1.\hspace{6pt}column:\hspace{6pt}channel\hspace{6pt}numbers;}}\\
{\it{\%\hspace{18pt}2.\hspace{6pt}column:\hspace{6pt}atomic\hspace{6pt}mass\hspace{6pt}units;\hspace{6pt}3.\hspace{6pt}column:\hspace{6pt}counts;}}\\
{\it{\%\hspace{18pt}masses\hspace{6pt}with\hspace{6pt}zero\hspace{6pt}counts\hspace{6pt}are\hspace{6pt}not\hspace{6pt}exported}}\\
{\it{\%m:\hspace{6pt}highest\hspace{6pt}mass\hspace{6pt}extracted}}\\
{\it{\%filled:\hspace{6pt}(mx1)\dash{}vector:\hspace{6pt}counts\hspace{6pt}for\hspace{6pt}m\hspace{6pt}masses}}\\

\\
c=0;
\\
go=1;
\\
k=1;
\\
\\
{\it{\%delete\hspace{6pt}first\hspace{6pt}row\hspace{6pt}if\hspace{6pt}it\hspace{6pt}contains\hspace{6pt}mass\hspace{6pt}0:
}}\\
{\textbf{if}}\hspace{6pt}in(1,2)==0
\\
\hspace{24pt}in=in(2:m+1,:);
\\
{\textbf{end}}
\\
\\
{\it{\%if\hspace{6pt}the\hspace{6pt}mass\hspace{6pt}spectrum\hspace{6pt}is\hspace{6pt}complete,}}\\
{\it{\%no\hspace{6pt}masses\hspace{6pt}with\hspace{6pt}0\hspace{6pt}counts\hspace{6pt}must\hspace{6pt}be\hspace{6pt}added:
}}\\
{\textbf{if}}\hspace{6pt}in(m,2)==m
\\
\hspace{24pt}go=0;
\\
\hspace{24pt}filled(:,1)=in(1:m,3);
\\
{\textbf{end}}
\\

\\
{\it{\%add\hspace{6pt}masses\hspace{6pt}with\hspace{6pt}0\hspace{6pt}counts:}}\\
{\it{\%loop\hspace{6pt}for\hspace{6pt}different\hspace{6pt}masses:
}}\\
{\textbf{while}}\hspace{6pt}go==1\\
\\
\hspace{24pt}{\it{\%check\hspace{6pt}if\hspace{6pt}mass\hspace{6pt}and\hspace{6pt}row\hspace{6pt}number\hspace{6pt}match}}\\
\hspace{24pt}{\it{\%and\hspace{6pt}add\hspace{6pt}the\hspace{6pt}missing\hspace{6pt}mass\hspace{6pt}if\hspace{6pt}they\hspace{6pt}do\hspace{6pt}not:
}}\\
\hspace{24pt}{\textbf{if}}\hspace{6pt}in(k\dash{}c,2)\~{}=k
\\
\hspace{48pt}filled(k,1)=0;\\
\hspace{48pt}{\it{\%c\hspace{6pt}accounts\hspace{6pt}for\hspace{6pt}the\hspace{6pt}shift\hspace{6pt}induced\hspace{6pt}by\hspace{6pt}adding\hspace{6pt}masses:
}}\\
\hspace{48pt}c=c+1;
\\
\hspace{24pt}{\textbf{else}}\hspace{6pt}
\\
\hspace{48pt}filled(k,1)=in(k\dash{}c,3);
\\
\hspace{24pt}{\textbf{end}}\\
\\
\hspace{24pt}{\it{\%stop\hspace{6pt}when\hspace{6pt}highest\hspace{6pt}mass\hspace{6pt}is\hspace{6pt}reached:
}}\\
\hspace{24pt}{\textbf{if}}\hspace{6pt}k==m
\\
\hspace{48pt}go=0;
\\
\hspace{24pt}{\textbf{end}}
\\
\hspace{24pt}k=k+1;
\\
{\textbf{end}}
\end{tabbing}}}


==> zuordnen.tex <==
{{\def\dash{\raise2.1pt\hbox{\rule{5pt}{0.3pt}}\hspace{1pt}}\begin{tabbing}
{\textbf{function}}\hspace{6pt}zuordnung=zuordnen(score,loading,intvar,anz,rep,data,dimmax)\\
{\it{\%zuordnung=zuordnen(score,loading,intvar,anz,rep,data,dimmax)}}\\
{\it{\%assigns\hspace{6pt}new\hspace{6pt}measurements\hspace{6pt}to\hspace{6pt}a\hspace{6pt}group\hspace{6pt}of\hspace{6pt}measurements}}\\
{\it{\%by\hspace{6pt}the\hspace{6pt}euclidean\hspace{6pt}distance\hspace{6pt}of\hspace{6pt}the\hspace{6pt}projection\hspace{6pt}into\hspace{6pt}the}}\\
{\it{\%DPC\hspace{6pt}space\hspace{6pt}calculated\hspace{6pt}with\hspace{6pt}the\hspace{6pt}original\hspace{6pt}measurements\hspace{6pt}to\hspace{6pt}the\hspace{6pt}}}\\
{\it{\%centers\hspace{6pt}of\hspace{6pt}gravity\hspace{6pt}of\hspace{6pt}the\hspace{6pt}original\hspace{6pt}groups}}\\
{\it{\%anz:\hspace{6pt}number\hspace{6pt}of\hspace{6pt}groups}}\\
{\it{\%rep:\hspace{6pt}(1xanz)\dash{}vector:\hspace{6pt}number\hspace{6pt}of\hspace{6pt}measurements\hspace{6pt}per\hspace{6pt}group}}\\
{\it{\%loading:\hspace{6pt}(mxm)\dash{}matrix:\hspace{6pt}loadings\hspace{6pt}of\hspace{6pt}m\hspace{6pt}DPC\hspace{6pt}as\hspace{6pt}m\hspace{6pt}columns}}\\
{\it{\%score:\hspace{6pt}(mxn)\dash{}matrix:\hspace{6pt}scores\hspace{6pt}of\hspace{6pt}m\hspace{6pt}DPC\hspace{6pt}for\hspace{6pt}n\hspace{6pt}measurements}}\\
{\it{\%intvar:\hspace{6pt}(mx1)\dash{}vector:\hspace{6pt}pooled\hspace{6pt}intra\hspace{6pt}group\hspace{6pt}variances\hspace{6pt}of\hspace{6pt}m\hspace{6pt}variables}}\\
{\it{\%dimmax:\hspace{6pt}dimensionality\hspace{6pt}of\hspace{6pt}the\hspace{6pt}DPC\hspace{6pt}space}}\\
{\it{\%zuordnung:\hspace{6pt}(nx(anz+1))\dash{}matrix:\hspace{6pt}first\hspace{6pt}column:\hspace{6pt}number\hspace{6pt}of\hspace{6pt}the\hspace{6pt}}}\\
{\it{\%\hspace{66pt}closest\hspace{6pt}group\hspace{6pt}to\hspace{6pt}a\hspace{6pt}measurement;\hspace{6pt}2.,3.,...\hspace{6pt}column:\hspace{6pt}}}\\
{\it{\%\hspace{66pt}relative\hspace{6pt}distance\hspace{6pt}to\hspace{6pt}the\hspace{6pt}1.,2.,...\hspace{6pt}group}}\\
\\
{[}m,n{]}=size(data);\\
{[}sizerepx,sizerepy{]}=size(rep);\\
{\textbf{if}}\hspace{6pt}sizerepy==1\\
\hspace{24pt}rep=repmat(rep,1,anz);\\
{\textbf{end}}\\
\\
{\it{\%DPCA\hspace{6pt}projection\hspace{6pt}of\hspace{6pt}the\hspace{6pt}new\hspace{6pt}data:}}\\
newscore=dpcaprojektion(loading,intvar,data,1,{\texttt{{'}no{'}}});\\
\\
{\it{\%loop\hspace{6pt}for\hspace{6pt}different\hspace{6pt}new\hspace{6pt}measurements\hspace{24pt}}}\\
\hspace{6pt}{\textbf{for}}\hspace{6pt}j=1:n\\
\hspace{30pt}\\
\hspace{30pt}{\it{\%select\hspace{6pt}one\hspace{6pt}measurement:}}\\
\hspace{30pt}newscorej=newscore(:,j);\\
\hspace{30pt}\\
\hspace{48pt}min=1;\\
\hspace{48pt}max=0;\\
\hspace{48pt}\\
\hspace{48pt}{\it{\%loop\hspace{6pt}for\hspace{6pt}different\hspace{6pt}groups:}}\\
\hspace{48pt}{\textbf{for}}\hspace{6pt}i=1:anz\\
\hspace{72pt}max=max+rep(i);\\
\\
\hspace{72pt}{\it{\%center\hspace{6pt}of\hspace{6pt}gravity\hspace{6pt}of\hspace{6pt}the\hspace{6pt}group:}}\\
\hspace{72pt}groupmean=mean(score(1:dimmax,min:max),2);\\
\\
\hspace{72pt}{\it{\%calculate\hspace{6pt}euclidean\hspace{6pt}distance:}}\\
\hspace{72pt}distance(i)=0;\\
\hspace{72pt}{\textbf{for}}\hspace{6pt}h=1:dimmax\\
\hspace{96pt}distance(i)=distance(i)+(newscorej(h)\dash{}groupmean(h))\^{}2;\\
\hspace{72pt}{\textbf{end}}\\
\hspace{72pt}distance(i)=sqrt(distance(i));\\
\hspace{72pt}min=min+rep(i);\\
\hspace{48pt}{\textbf{end}}\\
\hspace{48pt}\\
\hspace{48pt}{\it{\%assign\hspace{6pt}new\hspace{6pt}measurement\hspace{6pt}to\hspace{6pt}closest\hspace{6pt}group:}}\\
\hspace{48pt}{[}minimum,minimumindex{]}=min(distance);\\
\hspace{48pt}zuordnung(j,1)=minimumindex;\\
\\
\hspace{48pt}{\it{\%calculate\hspace{6pt}relative\hspace{6pt}distances\hspace{6pt}to\hspace{6pt}other\hspace{6pt}groups:}}\\
\hspace{48pt}{\textbf{for}}\hspace{6pt}i=1:anz\\
\hspace{72pt}zuordnung(j,1+i)=distance(i)/minimum;\\
\hspace{48pt}{\textbf{end}}\\
\hspace{24pt}{\textbf{end}}
\end{tabbing}}}
